Modeling and Performance Analysis of Pull-Based Live Streaming Schemes in Peer-to-Peer Network

Recent years mesh-based Peer-to-Peer live streaming has become a promising way for service providers to offer high-quality live video streaming service to Internet users. In this paper, we make a detailed study on modeling and performance analysis of the pull-based P2P streaming systems. We establish the analytical framework for the pull-based streaming schemes in P2P network, give accurate models of the chunk selection and peer selection strategies, and organize them into three categories, i.e., the chunk first scheme, the peer first scheme and the epidemic scheme. Through numerical performance evaluation, the impacts of some important parameters, such as size of neighbor set, reply number, buffer size and so on are investigated. For the peer first and chunk first scheme, we show that the pull-based schemes do not perform as well as the push-based schemes when peers are limited to reply only one request in each time slot. When the reply number increases, the pull-based streaming schemes will reach close to optimal playout probability. As to the pull-based epidemic scheme, we find it has unexpected poor performance, which is significantly different from the push-based epidemic scheme. Therefore we propose a simple, efficient and easily deployed push-pull scheme which can significantly improve the playout probability.

==> config.tex <==
\setvolume{x}                             %for printing use only
\setyear{2012}                             %for printing use only
\setpagerange{1}{16}                    %for printing use only
\setheadauthor{J. Zhang et al.}          %for printing use only
\setissn{1229-2370} \setpubdate{March 2012} \setno{1}

\afterpage{\beginheader}                   %for printing use only

